A Systematic Approach to Constructing Families of Incremental Topology Control Algorithms Using Graph Transformation

In the communication systems domain, constructing and maintaining network topologies via topology control (TC) algorithms is an important cross-cutting research area. Network topologies are usually modeled using attributed graphs whose nodes and edges represent the network nodes and their interconnecting links. A key requirement of TC algorithms is to fulfill certain consistency and optimization properties to ensure a high quality of service. Still, few attempts have been made to constructively integrate these properties into the development process of TC algorithms. Furthermore, even though many TC algorithms share substantial parts (such as structural patterns or tie-breaking strategies), few works constructively leverage these commonalities and differences of TC algorithms systematically. In previous work, we addressed the constructive integration of consistency properties into the development process. We outlined a constructive, model-driven methodology for designing individual TC algorithms. Valid and high-quality topologies are characterized using declarative graph constraints; TC algorithms are specified using programmed graph transformation. We applied a well-known static analysis technique to refine a given TC algorithm in a way that the resulting algorithm preserves the specified graph constraints. In this paper, we extend our constructive methodology by generalizing it to support the specification of families of TC algorithms. To show the feasibility of our approach, we reneging six existing TC algorithms and develop e-kTC, a novel energy-efficient variant of the TC algorithm kTC. Finally, we evaluate a subset of the specified TC algorithms using a new tool integration of the graph transformation tool eMoflon and the Simonstrator network simulation framework.

==> cfg_draftsettings.tex <==
% see also:
% https://tex.stackexchange.com/questions/15604/how-to-speed-up-pdflatex-for-a-very-large-document-on-macos-x#
\pdfcompresslevel=0
\pdfobjcompresslevel=0

==> energy-aware_ktc.tex <==
\section{e-kTC: Energy-Aware kTC}
\label{sec:ektc}
In the previous sections, we have demonstrated the top-down development methodology in detail for the \TC algorithm \ktc.
In this section, we will see why it may be beneficial for a \TC algorithm to take the remaining energy of the nodes into account when deciding which links to inactivate.
In \Cref{sec:metamodel-ektc}, we extend the topology meta-model with energy-related attributes.
In \Cref{sec:motivation-ektc}, we illustrate that executing \ktc may lead to suboptimal decisions that may shorten the lifetime of a network.
Based on these observations, we propose a novel variant of the \ktc algorithm in \Cref{sec:constraints-ektc}: \emph{energy-aware kTC}, \ektc for short.
In \Cref{sec:preservation-of-lifetime-ektc}, we show that \ektc preserves the lifetime of a topology.
In \Cref{sec:rule-refinement-ekc}, we point out that all properties that have been shown for \ktc carry over to \ektc as well.




\subsection{Extended Topology Meta-Model and Additional Context Event Rules}
\label{sec:metamodel-ektc}

To be able to describe energy-related properties of topologies, we extend the meta-model as shown in \Cref{fig:metamodel-topology-extended}.
A node $n$ has a \emph{remaining energy} $w(n)$;
the symbol $w$ alludes to the physical unit \emph{work}.
A link $e$ has a \emph{required transmission power} $p(e)$, which represents the (minimum) transmission power that is required to reach its target node from its source node.
%
\begin{figure}
    \begin{center}
        \includegraphics[width=.8\textwidth]{figures/topology_metamodel_with_energy/fig.pdf}
    \end{center}
    \caption{Extended meta-model of network topologies}
    \label{fig:metamodel-topology-extended}
\end{figure}
%
Two new \CE rules describe modifications of the values of the additional attributes: the
\remainingEnergyModificationRuleLong and the  \requiredTransmissionPowerModificationRuleLong, shown in \Cref{fig:context-event-rules-ektc}.
Both rules are structurally similar to the \weightModificationRuleLong.
%
\begin{figure}
    \begin{center}
        \includegraphics[width=.8\textwidth]{figures/context-event-rules-ektc/fig.png}
    \end{center}
    \caption{\CE rules for modifying the value of energy-related attributes}
    \label{fig:context-event-rules-ektc}
\end{figure}

The \defTerm{expected remaining lifetime} $r(e)$ of a link~$e$ is the maximum amount of time that the source node node $n$ of link~$e$ may transmit with power $p(e)$:
\begin{align}\label{eq:expected-remaining-lifetime}
    r(e) := \frac{w(n)}{p(e)}
\end{align}

The battery of a node \emph{depletes}\defTermMargin{battery depletion}, which means that its remaining energy gradually decreases over time.
The \defTerm{lifetime of a node} is the time that it takes until its remaining energy equals to zero.
The \defTerm{expected remaining lifetime \expectedRemLifetimeOfNode{v} of a node $v$} is the minimal expected remaining lifetime of its outgoing active links:
\begin{align*}
    r(v) := \min_{e=(v,w) \in E: s(e) = \ACT} r(e)
\end{align*}
For example, the expected remaining lifetime of node \nodeName{5} in the right topology of \Cref{fig:ektc-example} is 7.5 time steps.
The \emph{expected remaining lifetime \expectedRemLifetimeOfNode{G} of a topology $G$} is the minimum expected lifetime of all its nodes:
\begin{align*}
    r(G) := \min_{v \in V(G)} r(v)
\end{align*}
This definition is obviously a conservative estimation of the real lifetime of a network.
In the literature, a number of different notions of the lifetime of a network are applied, \eg, based on the number of connected components or on the percentage of empty nodes, which have zero remaining lifetime.
An upper bound of the maximum possible lifetime of a topology may be estimated by assuming that each node only uses its outgoing link with the minimal required transmission power.


\subsection{Motivation of Energy-Aware Topology Control}
\label{sec:motivation-ektc}

\Cref{fig:ktc-example-with-energy-consumption} illustrates that \ktc inactivates links only based on their weight value may lead to an unfavorable distribution of the lifetime of nodes, especially if the initial remaining energy of the nodes is distributed unequally.
%
\begin{figure}
    \begin{center}
        \subcaptionbox{Initial topology\label{fig:ktc-example-with-energy-consumption-A} }[.32\textwidth]{\includegraphics[width=.32\textwidth]{figures/example-ktc-battery-depletion/fig-A.png}}
        \subcaptionbox{After executing \ktc ($k{=}2$)\label{fig:ktc-example-with-energy-consumption-B}}[.32\textwidth]{\includegraphics[width=.32\textwidth]{figures/example-ktc-battery-depletion/fig-B.png}}
        \subcaptionbox{After 12 time steps\label{fig:ktc-example-with-energy-consumption-C}}[.32\textwidth]{\includegraphics[width=.32\textwidth]{figures/example-ktc-battery-depletion/fig-C.png}}
        
    \end{center}
    \caption{Applying \ktc to the sample topology taking into account the remaining energy of nodes}
    \label{fig:ktc-example-with-energy-consumption}
\end{figure}
%
In this example, we assume a static topology, that is, the link weights remain fixed during the lifetime of the network, which requires only one execution of \ktc (\Cref{fig:ktc-example-with-energy-consumption-A}).
Each link is labeled with its required transmission power and its expected remaining lifetime.
In this example, the required transmission power is calculated as follows and the remaining lifetime is calculated according to \Cref{eq:expected-remaining-lifetime}:
\begin{align*}
    p(e) = \frac{1}{100} \cdot w(e)^2.
\end{align*}
Initially, \ktc is executed with $k{=}2$ (\Cref{fig:ktc-example-with-energy-consumption-B}).
To illustrate the effects of applying \ktc, we simulate the behavior of the network over a number of discrete time steps using the following artificial workload until the first node runs out of energy:
In each time step, the remaining energy of a node is decreased by the greatest required transmission power among all of its active outgoing links.
This workload emulates a protocol that lets every node emit a message to its farthest active neighbor in every time step.
For instance, in each time step, the remaining energy of node \nodeName{4} decreases by 9.
The example shows that \nodeNameLong{4} runs out of energy after 12 time steps (\Cref{fig:ktc-example-with-energy-consumption-C}).




\subsection{Constraints of \ektc}
\label{sec:constraints-ektc}
The problem of unbalanced energy consumption is well-known in the literature and a number of \TC algorithms have been proposed that explicitly take the remaining energy of nodes into account (e.g.,~\cite{XH12,KMD07}).
We propose \ektc, a variant of \ktc that has been inspired by \cite{XH12}, that does not operate on the weight but on the expected remaining lifetime of links.

We require that after executing \ektc, a link is inactive if and only if this link is part of a triangle in which it has the unique minimum expected remaining lifetime among the links in the triangle and if its expected remaining lifetime is at least $k$ times shorter than the maximum expected remaining lifetime of the other links in the triangle. More formally:
\begin{align*}
    s(e) = \INACT 
        & \;\Leftrightarrow\; e \text{ is in triangle with links } e_{2},e_{3} \\
        & \wedge\; r(e) < \min\left(r(e_2), r(e_3)\right) \\
        & \wedge\; r(e) \leq \frac{1}{k} \cdot \max\left(r(e_2), r(e_3)\right).
\end{align*}
By inverting the second and third inequality, we obtain the following, equivalent expression:
\begin{align*}
    s(e) = \INACT 
    & \;\Leftrightarrow\; e \text{ is in triangle with links } e_{2},e_{3} \\
    & \wedge\; \frac{1}{r(e)} > \max\left(\frac{1}{r(e_2)}, \frac{1}{r(e_3)}\right) \\
    & \wedge\; \frac{1}{r(e)} \geq k \cdot \min\left(\frac{1}{r(e_2)}, \frac{1}{r(e_3)}\right).
\end{align*}
With $w(e) = 1/r(e)$ the two constraints listed above are identical to the constraints of \ktc as introduced in \Cref{sec:constraints}.
Therefore, \ektc may be interpreted as a variant of \ktc with just a different computation of the weight attribute of links. 
As for the basic \ktc algorithm, this property may be transformed into two implications, one for active links and one for inactive links, which correspond to the \activeLinkConstraintEKTCLong and the \inactiveLinkConstraintKTCLong of \ektc, depicted in \Cref{fig:constraints-of-ektc}.
%
\begin{figure}
    \begin{center}
        \includegraphics[width=.7\textwidth]{figures/ektc-constraints/fig.png}
    \end{center}
    \caption{Inactive-link constraint \inactiveLinkConstraintEKTC and \activeLinkConstraintEKTCLong of \ektc}\label{fig:constraints-of-ektc}
\end{figure}

\subsection{Preservation of lifetime}
\label{sec:preservation-of-lifetime-ektc}

\Cref{fig:ektc-example} illustrates that applying \ektc to the sample topology prolongs the lifetime of the network.
The initial topology is shown in \Cref{fig:ektc-example-A}.
In contrast to the previous example, the expected remaining lifetime of a link changes in each time step.
This requires applying \ektc incrementally, \eg, after every time step.
To make this example comparable with the previous one, we execute \ektc only once in the beginning (again with $k=2$), as shown in \Cref{fig:ektc-example-B}.
In this example, opposite links may have different states, which is illustrated by splitting a link if necessary and by marking the link state at the corresponding end.
Comparing the final topologies of this and the previous example in \Cref{fig:ktc-example-with-energy-consumption} shows that
the remaining energy of node \nodeName{2} has decreased, but the remaining energy of node \nodeName{4} is now 96.
Applying \ektc has increased the lifetime of the network by 4 time steps.
In this example, the increased lifetime is also equal to the maximum lifetime, which is equal to the maximum lifetime of node \nodeName{5}. 
%
\begin{figure}
    \begin{center}
         \subcaptionbox{Initial topology\label{fig:ektc-example-A} }[.32\textwidth]{\includegraphics[width=.32\textwidth]{figures/example-ektc/fig-A.png}}
         \subcaptionbox{After executing \ektc ($k{=}2$)\label{fig:ektc-example-B}}[.32\textwidth]{\includegraphics[width=.32\textwidth]{figures/example-ektc/fig-B.png}}
         \subcaptionbox{After 12 time steps\label{fig:ektc-example-C}}[.32\textwidth]{\includegraphics[width=.32\textwidth]{figures/example-ektc/fig-C.png}}
    \end{center}
    \caption{Example of executing \ektc on the sample topology.}
    \label{fig:ektc-example}
\end{figure}
%
The following theorem generalizes the observations of the previous example.
\begin{theorem}[Preservation of lifetime]\label{thm:lifetime-preservation-ektc}
Let $G$ be a topology consisting only of active links, and let $G_{\ektc}$ be the topology that results from unclassifying all links in $G$ and then applying \ektc.
Then, the expected remaining lifetime of $G_{\ektc}$ is at least as long as the expected remaining lifetime of $G$.
\end{theorem}
\begin{proof-sketch}
We prove for each node that its expected remaining lifetime in $G_{\ektc}$ is not less than its expected remaining lifetime in $G$.
All active links in $G_{\ektc}$ are also active in $G$.
Therefore it suffices to only consider the inactive links in $G_{\ektc}$ and to show for each inactive link that activating it would not increase the lifetime.

Let $s$ be some node in $G_{\ektc}$ and let $e$ be some inactive outgoing link of $s$.
The topology $G_{\ektc}$ fulfills the constraints of \ektc, and, therefore, $e$ is part of a triangle together with links $e_2$ and $e_3$ and 
\begin{align*}
\frac{1}{r(e)} > \max\left(\frac{1}{r(e_2)}, \frac{1}{r(e_3)}\right) 
\Leftrightarrow r(e) < \min\left(r(e_2), r(e_3)\right).
\end{align*}
This means that the expected remaining lifetime of $s$ would not increase if $e$ would be active.

This claim holds for all nodes in $G_{\ektc}$, including the node with the minimal remaining lifetime in $G_{\ektc}$, and therefore, the expected remaining lifetime of $G$ cannot be greater than the expected remaining lifetime of $G_{\ektc}$.
\end{proof-sketch}
Note that this theorem may only hold in a real application scenario if the required transmission power of a link is set to the power that is indeed required for reaching the target node from the source node, which is sometimes difficult to determine.

\subsection{Rule Refinement of TC and CE rules}
\label{sec:rule-refinement-ekc}

As the constraints of \ektc are equivalent to the constraints of \ktc using the modified weight attribute $w(e) = 1/r(e)$, the refinement of the \TC and the \CE rules is completely analogous to the steps described in \Cref{sec:refinement-of-tc-rules-with-active-constraint} to \Cref{sec:refinement-of-ce-rules-with-inactive-constraint}.
The refined rules for \ektc may be obtained by syntactically replacing $w(e)$ by $1/r(e)$ for each link variable $e$.
For the same reason, the proved properties of the \TC and \CE rules (termination of \TC, strong consistency after applying \TC, preservation of strong and weak connectivity) carry over to \ektc.


==> evaluation_lifetime.tex <==
\subsection{Research Question 2: Network Lifetime}
\label{sec:evaluation-rq2}
\paragraph{Results}
In \Cref{sec:ektc}, we defined the network lifetime as the minimum lifetime of its nodes.
We proved that executing e-kTC does not reduce the lifetime of the network under this assumption and the (core) assumption that the required transmission power of each link is the power that is necessary for reaching its target node from its source node.
However, in a realistic scenario, a \WSN is still usable if a relatively small fraction of the nodes runs out of energy.
The results of the neighboring nodes may substitute for the empty node.
In this respect, the number of nodes that may still transmit data to the base station is a salient metric for evaluating the lifetime of a network.

Therefore, for each configuration, we not only determined the point in time when the first node runs out of energy but also recorded the number of nodes that have a path to the base station in the physical topology.

\Cref{tab:evaluation-time-of-first-empty-node} shows for each configuration at which time during the simulation the first node runs out of energy.
\Cref{fig:evaluation-nodes-reachable-from-basestation} shows the number of nodes that are connected to the base station depending on the simulation time for the configurations with \numprint{50}, \numprint{250}, and \numprint{1000} nodes.%
%
\begin{table}
\begin{center}
    \caption{Point in time of first node failure due to empty battery}
    \label{tab:evaluation-time-of-first-empty-node}
    \begin{tabular}{l|ccc}
        \toprule
        \textbf{Configuration} & \textbf{No TC} & \textbf{\ktc} & \textbf{e-kTC}\\
        \midrule
        n=50,   size=100   &384&236&248\\
        n=125,  size=250	&321&154&170\\
        n=250,  size=500	&237& 87&101\\
        n=500,  size=1000	&109& 50& 71\\
        n=1000, size=2000	& 33& 27& 39\\
        \bottomrule
    \end{tabular}
\end{center}
\end{table}
%
\begin{figure}
\begin{center}
    \subcaptionbox%
    {n=50, size=100}[.95\textwidth]%
    {\includegraphics[width=.95\textwidth]{./figures/evaluation_plots/lifetime/network_lifetime__nodes_reachable_from_base_station_over_time_n050.pdf}}
    
%    \subcaptionbox{n=125, size=250}[.95\textwidth]{\includegraphics[width=.95\textwidth]{./figures/evaluation_plots/lifetime/network_lifetime__nodes_reachable_from_base_station_over_time_n125.pdf}}
    
    \subcaptionbox{n=250, size=500}[.95\textwidth]{\includegraphics[width=.95\textwidth]{./figures/evaluation_plots/lifetime/network_lifetime__nodes_reachable_from_base_station_over_time_n250.pdf}}
    
%    \subcaptionbox{n=500, size=1000}[\linewidth]{\includegraphics[width=\textwidth]{./figures/evaluation_plots/lifetime/network_lifetime__nodes_reachable_from_base_station_over_time_n500.pdf}}
    
    \subcaptionbox{n=1000, size=2000}[.95\linewidth]{\includegraphics[width=.95\textwidth]{./figures/evaluation_plots/lifetime/network_lifetime__nodes_reachable_from_base_station_over_time_n1000.pdf}}
    \caption{Number of nodes connected to the base station for each configuration (total simulation time: \SI{10}{\hour}=\SI{600}{\minute})}
    \label{fig:evaluation-nodes-reachable-from-basestation}
\end{center}
\end{figure}

\paragraph{Discussion}

The plots in \Cref{fig:evaluation-nodes-reachable-from-basestation} and \Cref{tab:evaluation-time-of-first-empty-node} show several remarkable particularities:
The smaller the average node degree is, the earlier is the point in time of the first node failure due to an empty battery, and most of the time, the unoptimized topology has the most nodes that may still reach the base station.
In this respect, \ktc performs worst, while e-kTC lies between the curves of not performing \TC and \ktc.
These results appear disappointing at first sight:
Not performing any kind of topology control is clearly the most favorable decision with respect to this metric in our evaluation.
In fact, these findings seem to contradict \Cref{thm:lifetime-preservation-ektc}, which claims that the network lifetime does not decrease when applying e-kTC.
In fact, the reason for this apparent contradiction is that we use different energy models for the simulation (WiFi chip BCM4329) and for making the decisions of e-kTC (Friis' transmission model), as explained above.
The data show that, at least, e-kTC is able to beat \ktc in terms of energy consumption for all configurations.

We argue that the effectiveness of \TC should be judged in relation to the application that runs on top of the optimized topology.
In this setting, none of the \TC algorithms could beat the baseline due to the fact that all data transmission nodes only send messages to a single base station and the underlying routing algorithm does already spend some efforts in selecting optimal routes to the base station even without \TC.
Deactivating links based on local (two hop context) knowledge only by e-kTC{}, cannot be expected to have a positive impact on the energy consumption of the nodes in this application scenario.
From this point of view, we selected a worst-case application scenario, which allows us to evaluate the incremental behavior of our TC algorithms (which is the focus of this paper!) under harsh conditions.

In contrast to the evaluation setup of this paper, the evaluation setup in~\cite{XH12}, which inspired us to develop e-kTC{}, studies a kind of best-case application scenario:
Each node in a topology sends in each round an individual message to each other node in the network (instead of sending only one message to the base station along a small range of possible routes).
In this case, the TC algorithm of~\cite{XH12}, which uses a similar optimization strategy as e-kTC{}, has a positive effect on the network lifetime.
We are, therefore, planning to implement new application scenarios in the \textsf{Simonstrator} platform that systematically cover the design space between best-case and worst-case scenarios as explained above. 
It was already noted in the literature that application-specific characteristics should be considered in \TC{} algorithms~\cite{Wang08,XLJP13}, and initial, promising results exist~\cite{KSSVMS14}.
\RY{004}{The results for the second RQ are surprising and disappointing, as it appears that not controlling the topology actually increases lifetime. As the reason for this lies in a mismatch between models, one would ask why this has not been taken into account before.}
\RX{040}{Section 7.4: I am not an expert in topology algorithms of ad-hoc networks, but this is not a very thorough evaluation of the algorithm. I think it lacks a systematic approach to ensure that your evaluation addresses typical situations and usual applications. After reading the evaluation, I know that in that single scenario I should not use the e-kTC algorithm but not when I can use it.}

==> evaluation_performance_tables.tex <==
\begin{table}[ht]
    \centering
    \caption{Algorithm performance for different weight thresholds \weightThreshold (world size: 500, node count: 99, $k = 1.00$).
        Lifetime values (\remainingLifetime{1}{}, \remainingLifetime{\SI{50}{\percent}}{}, \remainingLifetime{\SI{100}{\percent}}{}) are in simulated minutes. 
        Execution time $\overline{\executionTime{G_{\weightThreshold}}}$ is in CPU milliseconds.} 
    \label{tab:eval-chart-ws500-nc99-k1.00}
    \begin{tabular}{cr|rrrrrr}
        \toprule
        \multicolumn{1}{c}{\textbf{Algorithm}} & \multicolumn{1}{c|}{\textbf{\weightThreshold}} & \multicolumn{1}{c}{\textbf{\remainingLifetime{1}{} [min]}} & \multicolumn{1}{c}{\textbf{\relativeMetric{\remainingLifetime{1}{}}{}}} & \multicolumn{1}{c}{\textbf{\remainingLifetime{\SI{50}{\percent}}{} [min]}} & \multicolumn{1}{c}{\textbf{\relativeMetric{\remainingLifetime{\SI{50}{\percent}}{}}{}}} & \multicolumn{1}{c}{\textbf{\remainingLifetime{\SI{100}{\percent}}{} [min]}} & \multicolumn{1}{c}{\textbf{\relativeMetric{\remainingLifetime{\SI{100}{\percent}}{}}{}}} \\ 
        \midrule
        Maxpower & 0 & 564.0 & 1.00 & 700.0 & 1.00 & 854.0 & 1.00 \\ 
        \midrule
        kTC & 0 & 532.0 & 1.00 & 644.0 & 1.00 & 866.0 & 1.00 \\ 
        kTC & 20 & 538.0 & 1.01 & 652.0 & 1.01 & 864.0 & 1.00 \\ 
        kTC & 40 & 556.0 & 1.05 & 666.0 & 1.03 & 866.0 & 1.00 \\ 
        kTC & 60 & 574.0 & 1.08 & 684.0 & 1.06 & 870.0 & 1.00 \\ 
        kTC & 80 & 576.0 & 1.08 & 698.0 & 1.08 & 860.0 & 0.99 \\ 
        \midrule
        e-kTC & 0 & 626.0 & 1.00 & 754.0 & 1.00 & 890.0 & 1.00 \\ 
        e-kTC & 20 & 624.0 & 1.00 & 754.0 & 1.00 & 908.0 & 1.02 \\ 
        e-kTC & 40 & 606.0 & 0.97 & 730.0 & 0.97 & 886.0 & 1.00 \\ 
        e-kTC & 60 & 594.0 & 0.95 & 716.0 & 0.95 & 886.0 & 1.00 \\ 
        e-kTC & 80 & 584.0 & 0.93 & 708.0 & 0.94 & 864.0 & 0.97 \\ 
        \bottomrule
    \end{tabular}
    
    \centering
    \begin{tabular}{cr|rrrrrr}
        \toprule
        \multicolumn{1}{c}{\textbf{Algorithm}} & \multicolumn{1}{c|}{\textbf{\weightThreshold}} & \multicolumn{1}{c}{\textbf{$\overline{\cardinality{G_{\weightThreshold}}}$}} & \multicolumn{1}{c}{\textbf{\relativeTopologySize{}}} & \multicolumn{1}{c}{\textbf{$\overline{\executionTime{G_{\weightThreshold}}}$ [ms]}} & \multicolumn{1}{c}{\textbf{\relativeExecutionTime{}}} & \multicolumn{1}{c}{\textbf{$\overline{\lsmCount{G_{\weightThreshold}}}$}} & \multicolumn{1}{c}{\textbf{\relativeLSMCount{}}} \\ 
        \midrule
        Maxpower & 0 & 822.3 & 1.00 & 19.6 & 1.00 & 18.1 & 1.00 \\ 
        \midrule
        kTC & 0 & 751.6 & 1.00 & 232.2 & 1.00 & 1318.4 & 1.00 \\ 
        kTC & 20 & 753.3 & 1.00 & 228.6 & 0.98 & 1247.1 & 0.95 \\ 
        kTC & 40 & 746.5 & 0.99 & 165.8 & 0.71 & 1047.2 & 0.79 \\ 
        kTC & 60 & 698.5 & 0.93 & 111.2 & 0.48 & 801.1 & 0.61 \\ 
        kTC & 80 & 607.8 & 0.81 & 74.0 & 0.32 & 584.6 & 0.44 \\ 
        \midrule
        e-kTC & 0 & 902.8 & 1.00 & 316.5 & 1.00 & 1465.9 & 1.00 \\ 
        e-kTC & 20 & 894.5 & 0.99 & 302.9 & 0.96 & 1383.9 & 0.94 \\ 
        e-kTC & 40 & 826.0 & 0.91 & 201.3 & 0.64 & 1129.7 & 0.77 \\ 
        e-kTC & 60 & 738.3 & 0.82 & 129.3 & 0.41 & 839.3 & 0.57 \\ 
        e-kTC & 80 & 616.3 & 0.68 & 75.0 & 0.24 & 577.5 & 0.39 \\ 
        \bottomrule
    \end{tabular}
\end{table}
\begin{table}[ht]
    \centering
    \caption{Algorithm performance for different weight thresholds \weightThreshold (world size: 500, node count: 99, $k = 1.41$).
        Lifetime values (\remainingLifetime{1}{}, \remainingLifetime{\SI{50}{\percent}}{}, \remainingLifetime{\SI{100}{\percent}}{}) are in simulated minutes. 
        Execution time $\overline{\executionTime{G_{\weightThreshold}}}$ is in CPU milliseconds.} 
    \label{tab:eval-chart-ws500-nc99-k1.41}
    \begin{tabular}{cr|rrrrrr}
        \toprule
        \multicolumn{1}{c}{\textbf{Algorithm}} & \multicolumn{1}{c|}{\textbf{\weightThreshold}} & \multicolumn{1}{c}{\textbf{\remainingLifetime{1}{} [min]}} & \multicolumn{1}{c}{\textbf{\relativeMetric{\remainingLifetime{1}{}}{}}} & \multicolumn{1}{c}{\textbf{\remainingLifetime{\SI{50}{\percent}}{} [min]}} & \multicolumn{1}{c}{\textbf{\relativeMetric{\remainingLifetime{\SI{50}{\percent}}{}}{}}} & \multicolumn{1}{c}{\textbf{\remainingLifetime{\SI{100}{\percent}}{} [min]}} & \multicolumn{1}{c}{\textbf{\relativeMetric{\remainingLifetime{\SI{100}{\percent}}{}}{}}} \\ 
        \midrule
        Maxpower & 0 & 564.0 & 1.00 & 700.0 & 1.00 & 854.0 & 1.00 \\ 
        \midrule
        kTC & 0 & 544.0 & 1.00 & 664.0 & 1.00 & 862.0 & 1.00 \\ 
        kTC & 20 & 544.0 & 1.00 & 664.0 & 1.00 & 864.0 & 1.00 \\ 
        kTC & 40 & 570.0 & 1.05 & 684.0 & 1.03 & 868.0 & 1.01 \\ 
        kTC & 60 & 580.0 & 1.07 & 698.0 & 1.05 & 862.0 & 1.00 \\ 
        kTC & 80 & 564.0 & 1.04 & 702.0 & 1.06 & 860.0 & 1.00 \\ 
        \midrule
        e-kTC & 0 & 624.0 & 1.00 & 776.0 & 1.00 & 906.0 & 1.00 \\ 
        e-kTC & 20 & 624.0 & 1.00 & 770.0 & 0.99 & 902.0 & 1.00 \\ 
        e-kTC & 40 & 616.0 & 0.99 & 752.0 & 0.97 & 906.0 & 1.00 \\ 
        e-kTC & 60 & 600.0 & 0.96 & 726.0 & 0.94 & 882.0 & 0.97 \\ 
        e-kTC & 80 & 590.0 & 0.95 & 712.0 & 0.92 & 864.0 & 0.95 \\ 
        \bottomrule
    \end{tabular}
    
    \centering
    \begin{tabular}{cr|rrrrrr}
        \toprule
        \multicolumn{1}{c}{\textbf{Algorithm}} & \multicolumn{1}{c|}{\textbf{\weightThreshold}} & \multicolumn{1}{c}{\textbf{$\overline{\cardinality{G_{\weightThreshold}}}$}} & \multicolumn{1}{c}{\textbf{\relativeTopologySize{}}} & \multicolumn{1}{c}{\textbf{$\overline{\executionTime{G_{\weightThreshold}}}$ [ms]}} & \multicolumn{1}{c}{\textbf{\relativeExecutionTime{}}} & \multicolumn{1}{c}{\textbf{$\overline{\lsmCount{G_{\weightThreshold}}}$}} & \multicolumn{1}{c}{\textbf{\relativeLSMCount{}}} \\ 
        \midrule
        Maxpower & 0 & 822.3 & 1.00 & 19.8 & 1.00 & 18.1 & 1.00 \\ 
        \midrule
        kTC & 0 & 774.7 & 1.00 & 253.4 & 1.00 & 1340.3 & 1.00 \\ 
        kTC & 20 & 775.0 & 1.00 & 227.6 & 0.90 & 1252.2 & 0.93 \\ 
        kTC & 40 & 768.7 & 0.99 & 147.8 & 0.58 & 998.7 & 0.75 \\ 
        kTC & 60 & 712.7 & 0.92 & 83.1 & 0.33 & 728.0 & 0.54 \\ 
        kTC & 80 & 603.2 & 0.78 & 49.9 & 0.20 & 504.7 & 0.38 \\ 
        \midrule
        e-kTC & 0 & 927.4 & 1.00 & 240.7 & 1.00 & 1303.1 & 1.00 \\ 
        e-kTC & 20 & 912.9 & 0.98 & 211.6 & 0.88 & 1218.0 & 0.93 \\ 
        e-kTC & 40 & 853.5 & 0.92 & 151.8 & 0.63 & 1031.2 & 0.79 \\ 
        e-kTC & 60 & 747.3 & 0.81 & 115.8 & 0.48 & 791.2 & 0.61 \\ 
        e-kTC & 80 & 622.2 & 0.67 & 64.0 & 0.27 & 555.2 & 0.43 \\ 
        \bottomrule
    \end{tabular}
\end{table}
\begin{table}[ht]
    \centering
    \caption{Algorithm performance for different weight thresholds \weightThreshold (world size: 750, node count: 99, $k = 1.00$).
        Lifetime values (\remainingLifetime{1}{}, \remainingLifetime{\SI{50}{\percent}}{}, \remainingLifetime{\SI{100}{\percent}}{}) are in simulated minutes. 
        Execution time $\overline{\executionTime{G_{\weightThreshold}}}$ is in CPU milliseconds.} 
    \label{tab:eval-chart-ws750-nc99-k1.00}
    \begin{tabular}{cr|rrrrrr}
        \toprule
        \multicolumn{1}{c}{\textbf{Algorithm}} & \multicolumn{1}{c|}{\textbf{\weightThreshold}} & \multicolumn{1}{c}{\textbf{\remainingLifetime{1}{} [min]}} & \multicolumn{1}{c}{\textbf{\relativeMetric{\remainingLifetime{1}{}}{}}} & \multicolumn{1}{c}{\textbf{\remainingLifetime{\SI{50}{\percent}}{} [min]}} & \multicolumn{1}{c}{\textbf{\relativeMetric{\remainingLifetime{\SI{50}{\percent}}{}}{}}} & \multicolumn{1}{c}{\textbf{\remainingLifetime{\SI{100}{\percent}}{} [min]}} & \multicolumn{1}{c}{\textbf{\relativeMetric{\remainingLifetime{\SI{100}{\percent}}{}}{}}} \\ 
        \midrule
        Maxpower & 0 & 552.0 & 1.00 & 668.0 & 1.00 & 884.0 & 1.00 \\ 
        \midrule
        kTC & 0 & 518.0 & 1.00 & 632.0 & 1.00 & 898.0 & 1.00 \\ 
        kTC & 20 & 514.0 & 0.99 & 646.0 & 1.02 & 892.0 & 0.99 \\ 
        kTC & 40 & 524.0 & 1.01 & 646.0 & 1.02 & 878.0 & 0.98 \\ 
        kTC & 60 & 552.0 & 1.07 & 658.0 & 1.04 & 894.0 & 1.00 \\ 
        kTC & 80 & 556.0 & 1.07 & 668.0 & 1.06 & 890.0 & 0.99 \\ 
        \midrule
        e-kTC & 0 & 594.0 & 1.00 & 702.0 & 1.00 & 894.0 & 1.00 \\ 
        e-kTC & 20 & 598.0 & 1.01 & 714.0 & 1.02 & 908.0 & 1.02 \\ 
        e-kTC & 40 & 592.0 & 1.00 & 706.0 & 1.01 & 948.0 & 1.06 \\ 
        e-kTC & 60 & 572.0 & 0.96 & 692.0 & 0.99 & 916.0 & 1.02 \\ 
        e-kTC & 80 & 576.0 & 0.97 & 682.0 & 0.97 & 928.0 & 1.04 \\ 
        \bottomrule
    \end{tabular}
    
    \centering
    \begin{tabular}{cr|rrrrrr}
        \toprule
        \multicolumn{1}{c}{\textbf{Algorithm}} & \multicolumn{1}{c|}{\textbf{\weightThreshold}} & \multicolumn{1}{c}{\textbf{$\overline{\cardinality{G_{\weightThreshold}}}$}} & \multicolumn{1}{c}{\textbf{\relativeTopologySize{}}} & \multicolumn{1}{c}{\textbf{$\overline{\executionTime{G_{\weightThreshold}}}$ [ms]}} & \multicolumn{1}{c}{\textbf{\relativeExecutionTime{}}} & \multicolumn{1}{c}{\textbf{$\overline{\lsmCount{G_{\weightThreshold}}}$}} & \multicolumn{1}{c}{\textbf{\relativeLSMCount{}}} \\ 
        \midrule
        Maxpower & 0 & 412.9 & 1.00 & 9.6 & 1.00 & 9.0 & 1.00 \\ 
        \midrule
        kTC & 0 & 391.5 & 1.00 & 35.4 & 1.00 & 601.3 & 1.00 \\ 
        kTC & 20 & 394.8 & 1.01 & 33.5 & 0.95 & 574.6 & 0.96 \\ 
        kTC & 40 & 383.6 & 0.98 & 28.4 & 0.80 & 489.4 & 0.81 \\ 
        kTC & 60 & 363.3 & 0.93 & 24.6 & 0.69 & 391.7 & 0.65 \\ 
        kTC & 80 & 317.9 & 0.81 & 19.4 & 0.55 & 279.1 & 0.46 \\ 
        \midrule
        e-kTC & 0 & 441.8 & 1.00 & 39.1 & 1.00 & 635.2 & 1.00 \\ 
        e-kTC & 20 & 443.4 & 1.00 & 38.4 & 0.98 & 613.4 & 0.97 \\ 
        e-kTC & 40 & 424.5 & 0.96 & 34.3 & 0.88 & 529.1 & 0.83 \\ 
        e-kTC & 60 & 385.3 & 0.87 & 27.7 & 0.71 & 411.7 & 0.65 \\ 
        e-kTC & 80 & 327.4 & 0.74 & 22.2 & 0.57 & 283.6 & 0.45 \\ 
        \bottomrule
    \end{tabular}
\end{table}
\begin{table}[ht]
    \centering
    \caption{Algorithm performance for different weight thresholds \weightThreshold (world size: 750, node count: 99, $k = 1.41$).
        Lifetime values (\remainingLifetime{1}{}, \remainingLifetime{\SI{50}{\percent}}{}, \remainingLifetime{\SI{100}{\percent}}{}) are in simulated minutes. 
        Execution time $\overline{\executionTime{G_{\weightThreshold}}}$ is in CPU milliseconds.} 
    \label{tab:eval-chart-ws750-nc99-k1.41}
    \begin{tabular}{cr|rrrrrr}
        \toprule
        \multicolumn{1}{c}{\textbf{Algorithm}} & \multicolumn{1}{c|}{\textbf{\weightThreshold}} & \multicolumn{1}{c}{\textbf{\remainingLifetime{1}{} [min]}} & \multicolumn{1}{c}{\textbf{\relativeMetric{\remainingLifetime{1}{}}{}}} & \multicolumn{1}{c}{\textbf{\remainingLifetime{\SI{50}{\percent}}{} [min]}} & \multicolumn{1}{c}{\textbf{\relativeMetric{\remainingLifetime{\SI{50}{\percent}}{}}{}}} & \multicolumn{1}{c}{\textbf{\remainingLifetime{\SI{100}{\percent}}{} [min]}} & \multicolumn{1}{c}{\textbf{\relativeMetric{\remainingLifetime{\SI{100}{\percent}}{}}{}}} \\ 
        \midrule
        Maxpower & 0 & 552.0 & 1.00 & 668.0 & 1.00 & 884.0 & 1.00 \\ 
        \midrule
        kTC & 0 & 532.0 & 1.00 & 646.0 & 1.00 & 906.0 & 1.00 \\ 
        kTC & 20 & 532.0 & 1.00 & 650.0 & 1.01 & 942.0 & 1.04 \\ 
        kTC & 40 & 546.0 & 1.03 & 656.0 & 1.02 & 892.0 & 0.98 \\ 
        kTC & 60 & 554.0 & 1.04 & 670.0 & 1.04 & 894.0 & 0.99 \\ 
        kTC & 80 & 556.0 & 1.05 & 670.0 & 1.04 & 956.0 & 1.06 \\ 
        \midrule
        e-kTC & 0 & 592.0 & 1.00 & 710.0 & 1.00 & 958.0 & 1.00 \\ 
        e-kTC & 20 & 592.0 & 1.00 & 702.0 & 0.99 & 966.0 & 1.01 \\ 
        e-kTC & 40 & 590.0 & 1.00 & 696.0 & 0.98 & 902.0 & 0.94 \\ 
        e-kTC & 60 & 584.0 & 0.99 & 688.0 & 0.97 & 958.0 & 1.00 \\ 
        e-kTC & 80 & 574.0 & 0.97 & 684.0 & 0.96 & 944.0 & 0.99 \\ 
        \bottomrule
    \end{tabular}
    
    \centering
    \begin{tabular}{cr|rrrrrr}
        \toprule
        \multicolumn{1}{c}{\textbf{Algorithm}} & \multicolumn{1}{c|}{\textbf{\weightThreshold}} & \multicolumn{1}{c}{\textbf{$\overline{\cardinality{G_{\weightThreshold}}}$}} & \multicolumn{1}{c}{\textbf{\relativeTopologySize{}}} & \multicolumn{1}{c}{\textbf{$\overline{\executionTime{G_{\weightThreshold}}}$ [ms]}} & \multicolumn{1}{c}{\textbf{\relativeExecutionTime{}}} & \multicolumn{1}{c}{\textbf{$\overline{\lsmCount{G_{\weightThreshold}}}$}} & \multicolumn{1}{c}{\textbf{\relativeLSMCount{}}} \\ 
        \midrule
        Maxpower & 0 & 412.9 & 1.00 & 8.7 & 1.00 & 9.0 & 1.00 \\ 
        \midrule
        kTC & 0 & 401.5 & 1.00 & 36.5 & 1.00 & 604.9 & 1.00 \\ 
        kTC & 20 & 399.9 & 1.00 & 34.3 & 0.94 & 567.2 & 0.94 \\ 
        kTC & 40 & 390.8 & 0.97 & 27.7 & 0.76 & 473.4 & 0.78 \\ 
        kTC & 60 & 366.4 & 0.91 & 22.0 & 0.60 & 361.3 & 0.60 \\ 
        kTC & 80 & 319.7 & 0.80 & 17.6 & 0.48 & 245.3 & 0.41 \\ 
        \midrule
        e-kTC & 0 & 443.6 & 1.00 & 32.8 & 1.00 & 563.0 & 1.00 \\ 
        e-kTC & 20 & 435.9 & 0.98 & 31.5 & 0.96 & 532.9 & 0.95 \\ 
        e-kTC & 40 & 418.7 & 0.94 & 30.7 & 0.93 & 470.1 & 0.83 \\ 
        e-kTC & 60 & 383.8 & 0.87 & 25.8 & 0.79 & 383.2 & 0.68 \\ 
        e-kTC & 80 & 329.1 & 0.74 & 19.8 & 0.60 & 271.7 & 0.48 \\ 
        \bottomrule
    \end{tabular}
\end{table}

